An Efficient Application of Goal Programming to Tackle Multiobjective Problems with Recurring Fitness Landscapes

Many real-world applications require decision-makers to assess the quality of solutions while considering multiple conflicting objectives. Obtaining good approximation sets for highly constrained many-objective problems is often a difficult task even for modern multiobjective algorithms. In some cases, multiple instances of the problem scenario present similarities in their fitness landscapes. That is, there are recurring features in the fitness landscapes when searching for solutions to different problem instances. We propose a methodology to exploit this characteristic by solving one instance of a given problem scenario using computationally expensive multiobjective algorithms to obtain a good approximation set and then using Goal Programming with efficient single-objective algorithms to solve other instances of the same problem scenario. We use three goal-based objective functions and show that on benchmark instances of the multiobjective vehicle routing problem with time windows, the methodology is able to produce good results in short computation time. The methodology allows to combine the effectiveness of state-of-the-art multiobjective algorithms with the efficiency of goal programming to find good compromise solutions in problem scenarios where instances have similar fitness landscapes.

==> figures/api1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/api1}
    \caption{Overview of the API.}
    \label{fig:api1}
\end{figure}

==> figures/api2.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/api2}
    \caption{Main features of the WSRP API, where (1) refers to the optimisation solver (mathematical solver, heuristic algorithms, etc.), (2) and (10) to the data parser, (3) to the internal memory structures, (4) to (8) to the operations and methods supported by the API and (9) to the Solution Dispenser.}
    \label{fig:api2}
\end{figure*}

==> figures/diag0.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{figures/diag1}
    \caption{Class diagram for the main problem class and the tasks-related classes.}
    \label{fig:diag0}
\end{figure}

==> figures/sb.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/SB2}
    \caption{Flow diagram for the Solution Dispenser. Solid lines represent the flow for the 'New Solution' action, dashed lines for the 'Retrieve Solution' action and dotted lines for the 'Dispose Solution' action. }
    \label{fig:sb}
\end{figure*}

==> figures/step4.tex <==
\begin{figure*}
\centering
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-A}
\caption{Dataset A}
\label{mwsrp:step4a}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-B}
\caption{Dataset B}
\label{mwsrp:step4b}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-C}
\caption{Dataset C}
\label{mwsrp:step4c}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-D}
\caption{Dataset D}
\label{mwsrp:step4d}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-E}
\caption{Dataset E}
\label{mwsrp:step4e}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-F}
\caption{Dataset F}
\label{mwsrp:step4f}
\end{subfigure}
\caption{Scatter plots of each combined dataset, showing the relationship between objective $Z_4$ and each of the other four objectives. In each case, the $x$ axis shows the value of objective $Z_4$ and the $y$ axis shows the values of each of the other objectives in different colours.}
\label{mwsrp:step4}
\end{figure*}

==> figures/step4b.tex <==
\begin{figure*}
\centering
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-B-01}
\caption{Instance B1}
\label{mwsrp:step4a}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-B-03}
\caption{Instance B3}
\label{mwsrp:step4b}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-B-05}
\caption{Instance B5}
\label{mwsrp:step4c}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-D-01}
\caption{Instance D2}
\label{mwsrp:step4d}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-D-03}
\caption{Instance D4}
\label{mwsrp:step4e}
\end{subfigure}
\begin{subfigure}[t]{0.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/files/WSRP-D-05}
\caption{Instance D6}
\label{mwsrp:step4f}
\end{subfigure}
\caption{Scatter plots of three instances of datasets B and D. In each case, the $x$ axis shows the value of objective $Z_4$ and the $y$ axis shows the values of each of the other objectives in different colours.}
\label{mwsrp:step4}
\end{figure*}

==> sections/wsrp.tex <==
\section{The Workforce Scheduling and Routing Problem} \label{s2}

The WSRP is an optimisation problem that combines a scheduling and a routing problem. A set of $m$ workers $\{w_1, w_2, \dots, w_m\}$, must perform tasks on a set of $n$ visits $\{v_1, v_2, \dots, v_n\}$, which are distributed across distinct geographical locations. This work considers a specific case of this problem: the home healthcare planning problem, where workers are nurses, doctors and care workers and the purpose of the visits is to provide care to patients in their homes. For more information about this WSRP, please refer to \citet{Castillo2012,Castillo2014}.

The WSRP studied in this work contemplates the planning of a single day. Several hard constraints are considered in the problem: visits require a set of skills and only workers possessing the required skills can be assigned; workers can only be assigned to visits if allowed by their respective contracts; every visit must commence at a specified time in which workers must already be at the visits' premises; no time clashes are allowed, i.e. a worker cannot be assigned to simultaneous visits and there must be enough time for a worker to travel between visits. Also, two soft constraints are considered: workers may have a list of time intervals in which they are available; locations are grouped by geographical areas and workers may have a list of areas in which they are available. 

\input{figures/step4b}

The objectives considered in the problem are:
\begin{itemize}
    \item[$Z_1$] denotes the sum of the distances travelled by the workers, including commuting from their home to the first assignment, between each assignment, and from the final assignment back to their home; 
    \item[$Z_2$] denotes the sum of monetary assignment costs (workers wages for the assigned visits);
    \item[$Z_3$] denotes the sum of skill preferences in respect of assigning workers with skills that are desirable but not necessary;
    \item[$Z_4$] denotes the sum of patients preferences in respect of assigning preferred workers; and
    \item[$Z_5$] denotes the sum of workers preferences in respect of assigning workers to visits in their preferred area.
\end{itemize} 

Data from four different home healthcare companies of different sizes and characteristics was provided and six problem scenarios or dataset were generated. Each dataset (A, B, C, D, E and F) is composed of 7 instances for a total of 42 problem instances. Set A has small instances (number of visits and workers) while set F has the largest instances. 

Other works in the literature have also tackled the WSRP datasets considered here:
\begin{itemize}
    \item \cite{wasakorn} presented a computational study on the suitability of using exact methods to solve the problem. It was concluded that only the smaller instances can be solved to optimality by a mathematical solver. Later, \cite{wasakorn2} proposed to decompose the problem by geographical locations in order to employ the mathematical solver on the sub-problems and then use heuristic algorithms to integrate the partial solutions.
    \item \cite{haneen} conducted a study of various genetic operators applied to this problem. It was observed that the high number of constraints and large size of the instances presented a considerable challenge to the standard genetic algorithm implemented. Later, \cite{haneen2} proposed a knowledge-based indirect representation and genetic operators to improve the efficiency of the genetic algorithm for tackling the problem.
    \item More recently, \cite{Pinheiro2016} presented a Variable Neighbourhood Search (VNS) metaheuristic to tackle the WSRP, incorporating two novel heuristics tailored to the problem-domain. The first heuristic restricts the search space using a priority list of candidate workers and the second heuristic seeks to reduce the violation of specific soft constraints. Also, two greedy constructive heuristics were used to give the VNS a good starting point. Since that VNS is the best-known algorithm to tackle these WSRP instances, that algorithm is employed here within the proposed goal programming framework.
\end{itemize}

As preliminary work, we applied the analysis technique proposed by \citet{Pinheiro2015,Pinheiro2017} on all instances considered here. The technique consists of performing four steps: first the global pairwise relationships are analysed using the Kendall correlation method; then the ranges of the values found on the given approximation front are estimated and assessed; next these ranges are used to plot a map using Gray code, similar to Karnaugh maps, that has the ability to highlight the trade-offs between multiple objectives; and finally local relationships are identified using scatter plots. The conclusion is that in the studied datasets, instances of the same datset indeed present similar fitness landscapes. Figure \ref{mwsrp:step4} provides evidence of that and shows the scatter plots of instances B-01, B-03, B-05, D-02, D-04, and D-06 (arbitrarily chosen). Each datapoint corresponds to normalised objective values. For reasons of space, we omit the other datasets and the scatter plots of all instances. The resemblance between the fitness landscapes of the presented instances of datasets B and D is evident. Also, it is clear that different datasets present distinct fitness landscapes, even though they correspond to the same problem formulation. Finally, it is important to emphasise that datasets A, B and C present similar fitness landscapes with solutions well spread throughout the objective space while datasets D, E and F present distinct fitness landscapes with complex objective relationships and gaps. 



==> tables/wsrpinfo.tex <==
\begin{table*}
\centering
\caption{Basic information of the instances of each dataset.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{rlccccccccccccccccc}

\multicolumn{1}{l}{}             & \multicolumn{1}{l}{} & \multicolumn{8}{c}{\textbf{A}}                                                                                                                                                                                                                                                 & \multicolumn{1}{c}{\textbf{}} & \multicolumn{8}{c}{\textbf{B}}                                                                                                                                                                                                                                                 \\  
\multicolumn{1}{l}{}             & \multicolumn{1}{l}{} & \multicolumn{1}{c}{\textbf{01}} & \multicolumn{1}{c}{\textbf{02}} & \multicolumn{1}{c}{\textbf{03}} & \multicolumn{1}{c}{\textbf{04}} & \multicolumn{1}{c}{\textbf{05}} & \multicolumn{1}{c}{\textbf{06}} & \multicolumn{1}{c}{\textbf{07}} & \multicolumn{1}{c}{\textbf{mean}} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{01}} & \multicolumn{1}{c}{\textbf{02}} & \multicolumn{1}{c}{\textbf{03}} & \multicolumn{1}{c}{\textbf{04}} & \multicolumn{1}{c}{\textbf{05}} & \multicolumn{1}{c}{\textbf{06}} & \multicolumn{1}{c}{\textbf{07}} & \multicolumn{1}{c}{\textbf{mean}} \\ \cline{3-10} \cline{12-19} 
\textit{Number of Visits}         & \multicolumn{1}{l}{} & \multicolumn{1}{c}{31}          & \multicolumn{1}{c}{31}          & \multicolumn{1}{c}{38}          & \multicolumn{1}{c}{28}          & \multicolumn{1}{c}{13}          & \multicolumn{1}{c}{28}          & \multicolumn{1}{c}{13}          & \multicolumn{1}{c}{26}         & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{36}          & \multicolumn{1}{c}{12}          & \multicolumn{1}{c}{69}          & \multicolumn{1}{c}{30}          & \multicolumn{1}{c}{61}          & \multicolumn{1}{c}{57}          & \multicolumn{1}{c}{61}          & \multicolumn{1}{c}{46}         \\ 
\textit{Number of Workers}       & \multicolumn{1}{l}{} & \multicolumn{1}{c}{23}          & \multicolumn{1}{c}{22}          & \multicolumn{1}{c}{22}          & \multicolumn{1}{c}{19}          & \multicolumn{1}{c}{19}          & \multicolumn{1}{c}{21}          & \multicolumn{1}{c}{21}          & \multicolumn{1}{c}{21}         & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{25}          & \multicolumn{1}{c}{25}          & \multicolumn{1}{c}{34}          & \multicolumn{1}{c}{34}          & \multicolumn{1}{c}{32}          & \multicolumn{1}{c}{32}          & \multicolumn{1}{c}{32}          & \multicolumn{1}{c}{30}         \\ 
\textit{Number of Areas}         & \multicolumn{1}{l}{} & \multicolumn{1}{c}{5}           & \multicolumn{1}{c}{3}           & \multicolumn{1}{c}{4}           & \multicolumn{1}{c}{3}           & \multicolumn{1}{c}{3}           & \multicolumn{1}{c}{7}           & \multicolumn{1}{c}{3}           & \multicolumn{1}{c}{28}         & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{5}           & \multicolumn{1}{c}{4}           & \multicolumn{1}{c}{6}           & \multicolumn{1}{c}{4}           & \multicolumn{1}{c}{7}           & \multicolumn{1}{c}{7}           & \multicolumn{1}{c}{6}           & \multicolumn{1}{c}{5}          \\ 
\textit{Avg. Visit Duration (minutes)}      & \multicolumn{1}{l}{} & \multicolumn{1}{c}{144}         & \multicolumn{1}{c}{110}         & \multicolumn{1}{c}{102}         & \multicolumn{1}{c}{70}          & \multicolumn{1}{c}{57}          & \multicolumn{1}{c}{157}         & \multicolumn{1}{c}{104}         & \multicolumn{1}{c}{106}        & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{160}         & \multicolumn{1}{c}{155}         & \multicolumn{1}{c}{112}         & \multicolumn{1}{c}{58}          & \multicolumn{1}{c}{106}         & \multicolumn{1}{c}{101}         & \multicolumn{1}{c}{103}         & \multicolumn{1}{c}{113}        \\ \cline{3-10} \cline{12-19} 
\textit{}                        &                       &                                  &                                  &                                  &                                  &                                  &                                  &                                  &                                 &                                &                                  &                                  &                                  &                                  &                                  &                                  &                                  &                                 \\  
\multicolumn{1}{l}{}             & \multicolumn{1}{l}{} & \multicolumn{8}{c}{\textbf{C}}                                                                                                                                                                                                                                                 & \multicolumn{1}{c}{\textbf{}} & \multicolumn{8}{c}{\textbf{D}}                                                                                                                                                                                                                                                 \\ 
\multicolumn{1}{l}{}             & \multicolumn{1}{l}{} & \multicolumn{1}{c}{\textbf{01}} & \multicolumn{1}{c}{\textbf{02}} & \multicolumn{1}{c}{\textbf{03}} & \multicolumn{1}{c}{\textbf{04}} & \multicolumn{1}{c}{\textbf{05}} & \multicolumn{1}{c}{\textbf{06}} & \multicolumn{1}{c}{\textbf{07}} & \multicolumn{1}{c}{\textbf{mean}} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{01}} & \multicolumn{1}{c}{\textbf{02}} & \multicolumn{1}{c}{\textbf{03}} & \multicolumn{1}{c}{\textbf{04}} & \multicolumn{1}{c}{\textbf{05}} & \multicolumn{1}{c}{\textbf{06}} & \multicolumn{1}{c}{\textbf{07}} & \multicolumn{1}{c}{\textbf{mean}} \\ \cline{3-10} \cline{12-19} 
\textit{Number of Visits}         & \multicolumn{1}{l}{} & \multicolumn{1}{c}{177}         & \multicolumn{1}{c}{7}           & \multicolumn{1}{c}{150}         & \multicolumn{1}{c}{32}          & \multicolumn{1}{c}{29}          & \multicolumn{1}{c}{158}         & \multicolumn{1}{c}{6}           & \multicolumn{1}{c}{80}         & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{483}         & \multicolumn{1}{c}{454}         & \multicolumn{1}{c}{585}         & \multicolumn{1}{c}{520}         & \multicolumn{1}{c}{538}         & \multicolumn{1}{c}{610}         & \multicolumn{1}{c}{611}         & \multicolumn{1}{c}{543}        \\  
\textit{Number of Workers}       & \multicolumn{1}{l}{} & \multicolumn{1}{c}{1037}        & \multicolumn{1}{c}{618}         & \multicolumn{1}{c}{1077}        & \multicolumn{1}{c}{979}         & \multicolumn{1}{c}{821}         & \multicolumn{1}{c}{816}         & \multicolumn{1}{c}{349}         & \multicolumn{1}{c}{813}        & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{164}         & \multicolumn{1}{c}{166}         & \multicolumn{1}{c}{174}         & \multicolumn{1}{c}{174}         & \multicolumn{1}{c}{173}         & \multicolumn{1}{c}{174}         & \multicolumn{1}{c}{173}         & \multicolumn{1}{c}{171}        \\  
\textit{Number of Areas}         & \multicolumn{1}{l}{} & \multicolumn{1}{c}{7}           & \multicolumn{1}{c}{3}           & \multicolumn{1}{c}{6}           & \multicolumn{1}{c}{7}           & \multicolumn{1}{c}{5}           & \multicolumn{1}{c}{10}          & \multicolumn{1}{c}{5}           & \multicolumn{1}{c}{6}          & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{12}          & \multicolumn{1}{c}{11}          & \multicolumn{1}{c}{14}          & \multicolumn{1}{c}{14}          & \multicolumn{1}{c}{14}          & \multicolumn{1}{c}{14}          & \multicolumn{1}{c}{14}          & \multicolumn{1}{c}{13}         \\  
\textit{Avg. Visit Duration (minutes)}      & \multicolumn{1}{l}{} & \multicolumn{1}{c}{440}         & \multicolumn{1}{c}{599}         & \multicolumn{1}{c}{456}         & \multicolumn{1}{c}{356}         & \multicolumn{1}{c}{344}         & \multicolumn{1}{c}{469}         & \multicolumn{1}{c}{484}         & \multicolumn{1}{c}{449}        & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{62}          & \multicolumn{1}{c}{50}          & \multicolumn{1}{c}{67}          & \multicolumn{1}{c}{61}          & \multicolumn{1}{c}{58}          & \multicolumn{1}{c}{57}          & \multicolumn{1}{c}{56}          & \multicolumn{1}{c}{52}         \\  \cline{3-10} \cline{12-19} 
\multicolumn{1}{l}{}             &                       & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}            & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}            \\  
\textit{}                        & \multicolumn{1}{l}{} & \multicolumn{8}{c}{\textbf{E}}                                                                                                                                                                                                                                                 & \multicolumn{1}{c}{\textbf{}} & \multicolumn{8}{c}{\textbf{F}}                                                                                                                                                                                                                                                 \\  
\textit{}                        & \multicolumn{1}{l}{} & \multicolumn{1}{c}{\textbf{01}} & \multicolumn{1}{c}{\textbf{02}} & \multicolumn{1}{c}{\textbf{03}} & \multicolumn{1}{c}{\textbf{04}} & \multicolumn{1}{c}{\textbf{05}} & \multicolumn{1}{c}{\textbf{06}} & \multicolumn{1}{c}{\textbf{07}} & \multicolumn{1}{c}{\textbf{mean}} & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c}{\textbf{01}} & \multicolumn{1}{c}{\textbf{02}} & \multicolumn{1}{c}{\textbf{03}} & \multicolumn{1}{c}{\textbf{04}} & \multicolumn{1}{c}{\textbf{05}} & \multicolumn{1}{c}{\textbf{06}} & \multicolumn{1}{c}{\textbf{07}} & \multicolumn{1}{c}{\textbf{mean}} \\ \cline{3-10} \cline{12-19} 
\textit{Number of Visits}         & \multicolumn{1}{l}{} & \multicolumn{1}{c}{418}         & \multicolumn{1}{c}{425}         & \multicolumn{1}{c}{462}         & \multicolumn{1}{c}{351}         & \multicolumn{1}{c}{461}         & \multicolumn{1}{c}{301}         & \multicolumn{1}{c}{498}         & \multicolumn{1}{c}{416}        & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{1211}        & \multicolumn{1}{c}{1243}        & \multicolumn{1}{c}{1479}        & \multicolumn{1}{c}{1448}        & \multicolumn{1}{c}{1599}        & \multicolumn{1}{c}{1582}        & \multicolumn{1}{c}{1726}        & \multicolumn{1}{c}{1470}       \\ 
\textit{Number of Workers}       & \multicolumn{1}{l}{} & \multicolumn{1}{c}{243}         & \multicolumn{1}{c}{244}         & \multicolumn{1}{c}{267}         & \multicolumn{1}{c}{266}         & \multicolumn{1}{c}{278}         & \multicolumn{1}{c}{278}         & \multicolumn{1}{c}{302}         & \multicolumn{1}{c}{268}        & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{805}         & \multicolumn{1}{c}{769}         & \multicolumn{1}{c}{898}         & \multicolumn{1}{c}{789}         & \multicolumn{1}{c}{889}         & \multicolumn{1}{c}{783}         & \multicolumn{1}{c}{1011}        & \multicolumn{1}{c}{901}        \\  
\textit{Number of Areas}         & \multicolumn{1}{l}{} & \multicolumn{1}{c}{12}          & \multicolumn{1}{c}{13}          & \multicolumn{1}{c}{14}          & \multicolumn{1}{c}{12}          & \multicolumn{1}{c}{14}          & \multicolumn{1}{c}{12}          & \multicolumn{1}{c}{15}          & \multicolumn{1}{c}{13}         & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{44}          & \multicolumn{1}{c}{45}          & \multicolumn{1}{c}{53}          & \multicolumn{1}{c}{46}          & \multicolumn{1}{c}{58}          & \multicolumn{1}{c}{43}          & \multicolumn{1}{c}{63}          & \multicolumn{1}{c}{50}         \\ 
\textit{Avg. Visit Duration (minutes)}      & \multicolumn{1}{l}{} & \multicolumn{1}{c}{99}          & \multicolumn{1}{c}{102}         & \multicolumn{1}{c}{101}         & \multicolumn{1}{c}{73}          & \multicolumn{1}{c}{100}         & \multicolumn{1}{c}{64}          & \multicolumn{1}{c}{98}          & \multicolumn{1}{c}{91}         & \multicolumn{1}{c}{}          & \multicolumn{1}{c}{79}          & \multicolumn{1}{c}{87}          & \multicolumn{1}{c}{83}          & \multicolumn{1}{c}{89}          & \multicolumn{1}{c}{72}          & \multicolumn{1}{c}{81}          & \multicolumn{1}{c}{92}          & \multicolumn{1}{c}{83}         \\ 
 \cline{3-10} \cline{12-19} 
\textit{}                  &                       & \multicolumn{1}{l}{\textit{}}    & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}            & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}           
\end{tabular}
}
\label{table:wsrpinfo}
\end{table*}
